How Bayesian Should Bayesian Optimisation Be?

Bayesian optimisation (BO) uses probabilistic surrogate models - usually Gaussian processes (GPs) - for the optimisation of expensive black-box functions. At each BO iteration, the GP hyperparameters are fit to previously-evaluated data by maximising the marginal likelihood. However, this fails to account for uncertainty in the hyperparameters themselves, leading to overconfident model predictions. This uncertainty can be accounted for by taking the Bayesian approach of marginalising out the model hyperparameters. We investigate whether a fully-Bayesian treatment of the Gaussian process hyperparameters in BO (FBBO) leads to improved optimisation performance. Since an analytic approach is intractable, we compare FBBO using three approximate inference schemes to the maximum likelihood approach, using the Expected Improvement (EI) and Upper Confidence Bound (UCB) acquisition functions paired with ARD and isotropic Matern kernels, across 15 well-known benchmark problems for 4 observational noise settings. FBBO using EI with an ARD kernel leads to the best performance in the noise-free setting, with much less difference between combinations of BO components when the noise is increased. FBBO leads to over-exploration with UCB, but is not detrimental with EI. Therefore, we recommend that FBBO using EI with an ARD kernel as the default choice for BO.

==> includes/noise-free_ARD_ei.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{2pt}
\sisetup{table-format=1.2e-1, table-number-alignment=center}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l Sz Sz Sz Sz Sz}
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Branin (2)}
    & \multicolumn{2}{c}{\bfseries Eggholder (2)}
    & \multicolumn{2}{c}{\bfseries GoldsteinPrice (2)}
    & \multicolumn{2}{c}{\bfseries SixHumpCamel (2)}
    & \multicolumn{2}{c}{\bfseries Hartmann3 (3)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \statsimilar 1.93e-04 & \statsimilar 2.24e-04 &  \statsimilar 6.51e+01 & \statsimilar 5.22e+01 &  \best 2.17e-01 & \best 2.29e-01 &  \statsimilar 1.26e-04 & \statsimilar 1.65e-04 &  \statsimilar 9.52e-06 & \statsimilar 9.64e-06 \\
    MCMC &  \statsimilar 1.47e-04 & \statsimilar 1.68e-04 &  \best 3.19e+01 & \best 4.73e+01 &  \statsimilar 3.26e-01 & \statsimilar 4.32e-01 &  \statsimilar 1.64e-04 & \statsimilar 1.91e-04 &  \best 9.37e-06 & \best 1.06e-05 \\
    MFVI &  \statsimilar 1.04e-04 & \statsimilar 1.14e-04 &  6.57e+01 & 1.09e+00 &  \statsimilar 2.96e-01 & \statsimilar 3.46e-01 &  \best 1.00e-04 & \best 1.05e-04 &  \statsimilar 1.41e-05 & \statsimilar 1.67e-05 \\
    FRVI &  \best 8.98e-05 & \best 1.18e-04 &  \statsimilar 6.51e+01 & \statsimilar 1.37e+01 &  \statsimilar 3.16e-01 & \statsimilar 4.15e-01 &  1.85e-04 & 2.20e-04 &  \statsimilar 1.19e-05 & \statsimilar 1.35e-05 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Ackley5 (5)}
    & \multicolumn{2}{c}{\bfseries Michalewicz5 (5)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang5 (5)}
    & \multicolumn{2}{c}{\bfseries Hartmann6 (6)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock7 (7)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  2.33e+00 & 7.10e-01 &  \statsimilar 3.62e-01 & \statsimilar 4.04e-01 &  \statsimilar 6.40e+00 & \statsimilar 9.40e+00 &  2.82e-03 & 3.20e-03 &  2.86e+02 & 1.41e+02 \\
    MCMC &  \best 1.96e+00 & \best 6.40e-01 &  \best 2.41e-01 & \best 1.74e-01 &  \statsimilar 1.02e+00 & \statsimilar 1.35e+00 &  1.31e-03 & 1.57e-03 &  2.76e+02 & 1.50e+02 \\
    MFVI &  2.53e+00 & 3.84e-01 &  5.38e-01 & 4.20e-01 &  \statsimilar 9.44e-01 & \statsimilar 1.24e+00 &  \best 7.90e-04 & \best 9.55e-04 &  3.75e+02 & 2.21e+02 \\
    FRVI &  2.50e+00 & 4.51e-01 &  \statsimilar 3.90e-01 & \statsimilar 4.42e-01 &  \best 5.69e-01 & \best 5.21e-01 &  2.12e-03 & 2.70e-03 &  \best 2.07e+02 & \best 1.22e+02 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries StyblinskiTang7 (7)}
    & \multicolumn{2}{c}{\bfseries Ackley10 (10)}
    & \multicolumn{2}{c}{\bfseries Michalewicz10 (10)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock10 (10)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang10 (10)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \statsimilar 3.16e+01 & \statsimilar 1.71e+01 &  \statsimilar 3.59e+00 & \statsimilar 1.11e+00 &  3.57e+00 & 8.15e-01 &  \statsimilar 1.31e+03 & \statsimilar 5.56e+02 &  \statsimilar 7.57e+01 & \statsimilar 2.81e+01 \\
    MCMC &  \statsimilar 2.88e+01 & \statsimilar 1.91e+01 &  \statsimilar 3.52e+00 & \statsimilar 1.04e+00 &  \best 2.76e+00 & \best 7.34e-01 &  \statsimilar 1.35e+03 & \statsimilar 9.11e+02 &  \statsimilar 8.01e+01 & \statsimilar 2.71e+01 \\
    MFVI &  \statsimilar 3.34e+01 & \statsimilar 8.67e+00 &  \best 3.13e+00 & \best 3.96e-01 &  3.65e+00 & 7.43e-01 &  1.53e+03 & 5.76e+02 &  \statsimilar 7.49e+01 & \statsimilar 2.30e+01 \\
    FRVI &  \best 2.40e+01 & \best 1.32e+01 &  \statsimilar 3.19e+00 & \statsimilar 7.66e-01 &  \statsimilar 2.79e+00 & \statsimilar 9.08e-01 &  \best 1.14e+03 & \best 4.88e+02 &  \best 6.78e+01 & \best 1.73e+01 \\
\bottomrule
\end{tabular}
}%
\caption{Tabulated results for the EI acquisition function using an ARD kernel on the noise-free problems. The median log simple regret and the median absolute deviation from the median (MAD) is shown in the left- and right-hand columns respectively. The method with the lowest median performance is shown in dark grey, with those that are statistically equivalent shown in light grey.}
\label{tbl:ei:noise-free:ARD}
\end{table}

==> includes/noise-free_ARD_ucb.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{2pt}
\sisetup{table-format=1.2e-1, table-number-alignment=center}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l Sz Sz Sz Sz Sz}
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Branin (2)}
    & \multicolumn{2}{c}{\bfseries Eggholder (2)}
    & \multicolumn{2}{c}{\bfseries GoldsteinPrice (2)}
    & \multicolumn{2}{c}{\bfseries SixHumpCamel (2)}
    & \multicolumn{2}{c}{\bfseries Hartmann3 (3)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 2.98e-03 & \best 3.12e-03 &  \best 8.44e+01 & \best 2.73e+01 &  \statsimilar 1.88e+00 & \statsimilar 1.26e+00 &  \statsimilar 1.43e-03 & \statsimilar 1.29e-03 &  \best 9.75e-04 & \best 5.34e-04 \\
    MCMC &  6.10e-03 & 7.76e-03 &  \statsimilar 9.44e+01 & \statsimilar 4.78e+01 &  \statsimilar 2.66e+00 & \statsimilar 1.45e+00 &  \statsimilar 2.17e-03 & \statsimilar 2.41e-03 &  1.75e-03 & 4.76e-04 \\
    MFVI &  7.48e-03 & 9.78e-03 &  \statsimilar 9.26e+01 & \statsimilar 5.58e+01 &  \best 1.86e+00 & \best 1.88e+00 &  \best 1.33e-03 & \best 1.32e-03 &  1.92e-03 & 2.83e-04 \\
    FRVI &  5.87e-03 & 7.57e-03 &  \statsimilar 1.05e+02 & \statsimilar 4.96e+01 &  \statsimilar 1.93e+00 & \statsimilar 1.69e+00 &  \statsimilar 2.12e-03 & \statsimilar 1.92e-03 &  1.84e-03 & 3.21e-04 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Ackley5 (5)}
    & \multicolumn{2}{c}{\bfseries Michalewicz5 (5)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang5 (5)}
    & \multicolumn{2}{c}{\bfseries Hartmann6 (6)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock7 (7)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 3.73e+00 & \best 4.94e-01 &  \best 1.64e+00 & \best 4.85e-01 &  \best 4.72e+01 & \best 1.12e+01 &  \best 5.76e-03 & \best 5.15e-03 &  \best 9.12e+03 & \best 5.98e+03 \\
    MCMC &  4.86e+00 & 7.40e-01 &  2.09e+00 & 3.95e-01 &  5.51e+01 & 1.13e+01 &  3.98e-02 & 5.49e-02 &  1.68e+04 & 1.29e+04 \\
    MFVI &  5.02e+00 & 7.67e-01 &  2.12e+00 & 4.73e-01 &  5.42e+01 & 9.16e+00 &  1.60e-02 & 2.25e-02 &  1.79e+04 & 1.34e+04 \\
    FRVI &  4.87e+00 & 7.62e-01 &  2.11e+00 & 3.65e-01 &  5.42e+01 & 1.32e+01 &  4.03e-02 & 5.62e-02 &  1.59e+04 & 1.16e+04 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries StyblinskiTang7 (7)}
    & \multicolumn{2}{c}{\bfseries Ackley10 (10)}
    & \multicolumn{2}{c}{\bfseries Michalewicz10 (10)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock10 (10)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang10 (10)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 7.12e+01 & \best 1.34e+01 &  \best 6.05e+00 & \best 7.66e-01 &  \best 4.94e+00 & \best 3.91e-01 &  \best 1.32e+04 & \best 1.31e+04 &  \best 1.10e+02 & \best 2.37e+01 \\
    MCMC &  1.06e+02 & 2.09e+01 &  7.99e+00 & 1.03e+00 &  5.41e+00 & 6.20e-01 &  7.13e+04 & 1.98e+04 &  1.27e+02 & 2.69e+01 \\
    MFVI &  1.15e+02 & 1.62e+01 &  8.36e+00 & 1.23e+00 &  5.48e+00 & 5.30e-01 &  7.28e+04 & 2.27e+04 &  1.56e+02 & 3.00e+01 \\
    FRVI &  1.19e+02 & 1.94e+01 &  8.17e+00 & 9.96e-01 &  \statsimilar 5.14e+00 & \statsimilar 5.31e-01 &  7.15e+04 & 2.22e+04 &  \statsimilar 1.17e+02 & \statsimilar 1.88e+01 \\
\bottomrule
\end{tabular}
}%
\caption{Tabulated results for the UCB acquisition function using an ARD kernel on the noise-free problems. The median log simple regret and the median absolute deviation from the median (MAD) is shown in the left- and right-hand columns respectively. The method with the lowest median performance is shown in dark grey, with those that are statistically equivalent shown in light grey.}
\label{tbl:ucb:noise-free:ARD}
\end{table}

==> includes/noise-free_isotropic_ei.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{2pt}
\sisetup{table-format=1.2e-1, table-number-alignment=center}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l Sz Sz Sz Sz Sz}
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Branin (2)}
    & \multicolumn{2}{c}{\bfseries Eggholder (2)}
    & \multicolumn{2}{c}{\bfseries GoldsteinPrice (2)}
    & \multicolumn{2}{c}{\bfseries SixHumpCamel (2)}
    & \multicolumn{2}{c}{\bfseries Hartmann3 (3)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \statsimilar 1.05e-04 & \statsimilar 1.22e-04 &  \best 6.51e+01 & \best 4.83e+01 &  \statsimilar 4.27e-01 & \statsimilar 4.07e-01 &  \best 3.21e-05 & \best 4.00e-05 &  \statsimilar 4.91e-05 & \statsimilar 4.55e-05 \\
    MCMC &  1.68e-04 & 2.31e-04 &  \statsimilar 6.51e+01 & \statsimilar 1.06e+01 &  \best 3.42e-01 & \best 4.31e-01 &  1.30e-04 & 1.50e-04 &  8.30e-05 & 8.89e-05 \\
    MFVI &  \best 6.92e-05 & \best 8.19e-05 &  \statsimilar 6.58e+01 & \statsimilar 4.98e+00 &  \statsimilar 3.66e-01 & \statsimilar 3.84e-01 &  7.41e-05 & 8.48e-05 &  \best 4.23e-05 & \best 3.82e-05 \\
    FRVI &  1.74e-04 & 2.20e-04 &  \statsimilar 6.51e+01 & \statsimilar 5.57e+00 &  \statsimilar 3.78e-01 & \statsimilar 4.51e-01 &  6.75e-05 & 9.10e-05 &  1.00e-04 & 1.17e-04 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Ackley5 (5)}
    & \multicolumn{2}{c}{\bfseries Michalewicz5 (5)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang5 (5)}
    & \multicolumn{2}{c}{\bfseries Hartmann6 (6)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock7 (7)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 1.89e+00 & \best 1.51e+00 &  \best 8.21e-01 & \best 6.53e-01 &  \best 5.37e-01 & \best 6.21e-01 &  \statsimilar 4.30e-03 & \statsimilar 5.29e-03 &  \best 2.44e+02 & \best 1.38e+02 \\
    MCMC &  \statsimilar 2.08e+00 & \statsimilar 9.03e-01 &  \statsimilar 8.31e-01 & \statsimilar 5.64e-01 &  \statsimilar 6.15e-01 & \statsimilar 7.40e-01 &  \statsimilar 4.07e-03 & \statsimilar 5.18e-03 &  \statsimilar 2.57e+02 & \statsimilar 1.99e+02 \\
    MFVI &  \statsimilar 2.68e+00 & \statsimilar 5.92e-01 &  1.20e+00 & 5.52e-01 &  \statsimilar 3.72e+00 & \statsimilar 4.16e+00 &  \best 2.24e-03 & \best 2.38e-03 &  5.36e+02 & 3.41e+02 \\
    FRVI &  \statsimilar 2.71e+00 & \statsimilar 5.91e-01 &  1.11e+00 & 4.33e-01 &  \statsimilar 6.48e-01 & \statsimilar 7.13e-01 &  \statsimilar 4.98e-03 & \statsimilar 6.67e-03 &  \statsimilar 2.54e+02 & \statsimilar 1.74e+02 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries StyblinskiTang7 (7)}
    & \multicolumn{2}{c}{\bfseries Ackley10 (10)}
    & \multicolumn{2}{c}{\bfseries Michalewicz10 (10)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock10 (10)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang10 (10)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 2.86e+01 & \best 1.29e+01 &  1.24e+01 & 7.39e+00 &  5.33e+00 & 6.25e-01 &  \statsimilar 8.39e+02 & \statsimilar 4.22e+02 &  \statsimilar 7.18e+01 & \statsimilar 2.26e+01 \\
    MCMC &  \statsimilar 2.93e+01 & \statsimilar 1.79e+01 &  1.40e+01 & 5.15e+00 &  5.26e+00 & 6.87e-01 &  \best 7.52e+02 & \best 3.71e+02 &  \best 6.62e+01 & \best 2.91e+01 \\
    MFVI &  3.17e+01 & 1.27e+01 &  \best 3.11e+00 & \best 5.06e-01 &  \statsimilar 4.59e+00 & \statsimilar 8.53e-01 &  2.05e+03 & 8.47e+02 &  7.93e+01 & 2.70e+01 \\
    FRVI &  \statsimilar 2.87e+01 & \statsimilar 1.76e+01 &  3.51e+00 & 1.40e+00 &  \best 4.54e+00 & \best 7.33e-01 &  9.97e+02 & 4.73e+02 &  \statsimilar 7.24e+01 & \statsimilar 2.32e+01 \\
\bottomrule
\end{tabular}
}%
\caption{Tabulated results for the EI acquisition function using an isotropic kernel on the noise-free problems. The median log simple regret and the median absolute deviation from the median (MAD) is shown in the left- and right-hand columns respectively. The method with the lowest median performance is shown in dark grey, with those that are statistically equivalent shown in light grey.}
\label{tbl:ei:noise-free:isotropic}
\end{table}

==> includes/noise-free_isotropic_ucb.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{2pt}
\sisetup{table-format=1.2e-1, table-number-alignment=center}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l Sz Sz Sz Sz Sz}
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Branin (2)}
    & \multicolumn{2}{c}{\bfseries Eggholder (2)}
    & \multicolumn{2}{c}{\bfseries GoldsteinPrice (2)}
    & \multicolumn{2}{c}{\bfseries SixHumpCamel (2)}
    & \multicolumn{2}{c}{\bfseries Hartmann3 (3)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 1.69e-03 & \best 1.72e-03 &  \statsimilar 9.50e+01 & \statsimilar 2.96e+01 &  \best 1.56e+00 & \best 1.42e+00 &  \best 1.02e-03 & \best 1.23e-03 &  \best 6.09e-04 & \best 4.03e-04 \\
    MCMC &  3.90e-03 & 4.75e-03 &  \statsimilar 1.06e+02 & \statsimilar 3.48e+01 &  2.60e+00 & 1.88e+00 &  3.93e-03 & 3.84e-03 &  6.81e-04 & 5.78e-04 \\
    MFVI &  \statsimilar 2.68e-03 & \statsimilar 2.71e-03 &  \statsimilar 1.04e+02 & \statsimilar 5.15e+01 &  2.76e+00 & 2.06e+00 &  5.36e-03 & 4.83e-03 &  1.08e-03 & 7.36e-04 \\
    FRVI &  4.86e-03 & 5.21e-03 &  \best 8.55e+01 & \best 6.97e+01 &  1.85e+00 & 1.96e+00 &  4.86e-03 & 3.35e-03 &  7.76e-04 & 6.42e-04 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Ackley5 (5)}
    & \multicolumn{2}{c}{\bfseries Michalewicz5 (5)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang5 (5)}
    & \multicolumn{2}{c}{\bfseries Hartmann6 (6)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock7 (7)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 3.74e+00 & \best 5.42e-01 &  \best 1.15e+00 & \best 2.59e-01 &  \best 2.79e+01 & \best 8.73e+00 &  \best 8.94e-02 & \best 1.21e-01 &  \statsimilar 6.61e+03 & \statsimilar 4.81e+03 \\
    MCMC &  4.67e+00 & 1.02e+00 &  1.40e+00 & 2.67e-01 &  4.36e+01 & 6.22e+00 &  2.74e-01 & 1.16e-01 &  \best 4.30e+03 & \best 4.71e+03 \\
    MFVI &  5.08e+00 & 7.63e-01 &  1.42e+00 & 2.67e-01 &  4.23e+01 & 6.90e+00 &  3.05e-01 & 1.19e-01 &  \statsimilar 5.82e+03 & \statsimilar 5.49e+03 \\
    FRVI &  4.86e+00 & 9.71e-01 &  1.40e+00 & 4.06e-01 &  4.28e+01 & 8.43e+00 &  2.95e-01 & 1.51e-01 &  \statsimilar 4.34e+03 & \statsimilar 3.62e+03 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries StyblinskiTang7 (7)}
    & \multicolumn{2}{c}{\bfseries Ackley10 (10)}
    & \multicolumn{2}{c}{\bfseries Michalewicz10 (10)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock10 (10)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang10 (10)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 5.93e+01 & \best 1.01e+01 &  \best 5.94e+00 & \best 6.35e-01 &  \statsimilar 4.68e+00 & \statsimilar 4.53e-01 &  \best 2.21e+04 & \best 1.77e+04 &  \best 1.13e+02 & \best 2.33e+01 \\
    MCMC &  1.20e+02 & 2.24e+01 &  7.72e+00 & 1.07e+00 &  \statsimilar 4.87e+00 & \statsimilar 4.29e-01 &  6.30e+04 & 3.00e+04 &  1.44e+02 & 3.91e+01 \\
    MFVI &  1.24e+02 & 1.68e+01 &  7.25e+00 & 9.96e-01 &  \best 4.67e+00 & \best 7.75e-01 &  6.71e+04 & 1.58e+04 &  1.69e+02 & 4.60e+01 \\
    FRVI &  1.27e+02 & 1.78e+01 &  7.89e+00 & 1.01e+00 &  \statsimilar 4.82e+00 & \statsimilar 6.42e-01 &  6.01e+04 & 1.93e+04 &  1.96e+02 & 2.00e+01 \\
\bottomrule
\end{tabular}
}%
\caption{Tabulated results for the UCB acquisition function using an isotropic kernel on the noise-free problems. The median log simple regret and the median absolute deviation from the median (MAD) is shown in the left- and right-hand columns respectively. The method with the lowest median performance is shown in dark grey, with those that are statistically equivalent shown in light grey.}
\label{tbl:ucb:noise-free:isotropic}
\end{table}

==> includes/noise=0.05_ARD_ei.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{2pt}
\sisetup{table-format=1.2e-1, table-number-alignment=center}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l Sz Sz Sz Sz Sz}
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Branin (2)}
    & \multicolumn{2}{c}{\bfseries Eggholder (2)}
    & \multicolumn{2}{c}{\bfseries GoldsteinPrice (2)}
    & \multicolumn{2}{c}{\bfseries SixHumpCamel (2)}
    & \multicolumn{2}{c}{\bfseries Hartmann3 (3)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 4.20e-02 & \best 4.24e-02 &  \statsimilar 6.74e+01 & \statsimilar 6.89e+00 &  \best 4.24e+00 & \best 4.59e+00 &  \statsimilar 2.09e-02 & \statsimilar 2.67e-02 &  \best 5.99e-03 & \best 2.74e-03 \\
    MCMC &  \statsimilar 4.67e-02 & \statsimilar 4.87e-02 &  \best 6.64e+01 & \best 9.27e+00 &  \statsimilar 5.89e+00 & \statsimilar 5.42e+00 &  \best 2.09e-02 & \best 2.27e-02 &  \statsimilar 7.89e-03 & \statsimilar 3.81e-03 \\
    MFVI &  \statsimilar 5.43e-02 & \statsimilar 6.16e-02 &  \statsimilar 6.67e+01 & \statsimilar 7.33e+00 &  \statsimilar 6.69e+00 & \statsimilar 6.16e+00 &  \statsimilar 2.82e-02 & \statsimilar 3.06e-02 &  8.37e-03 & 2.14e-03 \\
    FRVI &  \statsimilar 6.47e-02 & \statsimilar 6.07e-02 &  \statsimilar 6.67e+01 & \statsimilar 6.67e+00 &  \statsimilar 5.49e+00 & \statsimilar 5.47e+00 &  \statsimilar 2.76e-02 & \statsimilar 2.86e-02 &  \statsimilar 8.25e-03 & \statsimilar 4.69e-03 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Ackley5 (5)}
    & \multicolumn{2}{c}{\bfseries Michalewicz5 (5)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang5 (5)}
    & \multicolumn{2}{c}{\bfseries Hartmann6 (6)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock7 (7)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \statsimilar 6.40e+00 & \statsimilar 1.96e+00 &  1.77e+00 & 4.55e-01 &  \best 3.38e+01 & \best 1.43e+01 &  \statsimilar 8.41e-02 & \statsimilar 7.47e-02 &  4.74e+03 & 2.78e+03 \\
    MCMC &  \best 5.97e+00 & \best 2.00e+00 &  \best 1.29e+00 & \best 3.19e-01 &  4.32e+01 & 1.51e+01 &  \statsimilar 8.07e-02 & \statsimilar 6.57e-02 &  \best 2.00e+03 & \best 1.38e+03 \\
    MFVI &  7.57e+00 & 1.96e+00 &  1.71e+00 & 3.62e-01 &  4.66e+01 & 1.64e+01 &  \best 7.83e-02 & \best 6.71e-02 &  \statsimilar 2.19e+03 & \statsimilar 1.14e+03 \\
    FRVI &  \statsimilar 6.14e+00 & \statsimilar 1.93e+00 &  1.71e+00 & 3.97e-01 &  4.36e+01 & 1.30e+01 &  \statsimilar 7.93e-02 & \statsimilar 6.31e-02 &  \statsimilar 2.32e+03 & \statsimilar 1.38e+03 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries StyblinskiTang7 (7)}
    & \multicolumn{2}{c}{\bfseries Ackley10 (10)}
    & \multicolumn{2}{c}{\bfseries Michalewicz10 (10)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock10 (10)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang10 (10)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 6.44e+01 & \best 1.85e+01 &  \best 1.51e+01 & \best 3.53e+00 &  \statsimilar 5.23e+00 & \statsimilar 5.46e-01 &  9.05e+03 & 4.82e+03 &  \best 1.18e+02 & \best 2.15e+01 \\
    MCMC &  \statsimilar 6.99e+01 & \statsimilar 2.55e+01 &  \statsimilar 1.71e+01 & \statsimilar 2.70e+00 &  \best 5.09e+00 & \best 8.41e-01 &  \statsimilar 5.65e+03 & \statsimilar 3.55e+03 &  \statsimilar 1.26e+02 & \statsimilar 2.16e+01 \\
    MFVI &  7.86e+01 & 1.61e+01 &  1.72e+01 & 3.16e+00 &  \statsimilar 5.21e+00 & \statsimilar 7.65e-01 &  \best 4.77e+03 & \best 2.95e+03 &  \statsimilar 1.21e+02 & \statsimilar 2.69e+01 \\
    FRVI &  7.78e+01 & 1.82e+01 &  \statsimilar 1.53e+01 & \statsimilar 5.31e+00 &  \statsimilar 5.23e+00 & \statsimilar 4.12e-01 &  \statsimilar 5.30e+03 & \statsimilar 2.56e+03 &  \statsimilar 1.24e+02 & \statsimilar 3.18e+01 \\
\bottomrule
\end{tabular}
}%
\caption{Tabulated results for the EI acquisition function using an ARD kernel on the $\sigma_n = 0.05$ problems. The median log simple regret and the median absolute deviation from the median (MAD) is shown in the left- and right-hand columns respectively. The method with the lowest median performance is shown in dark grey, with those that are statistically equivalent shown in light grey.}
\label{tbl:ei:noise=0.05:ARD}
\end{table}

==> includes/noise=0.05_ARD_ucb.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{2pt}
\sisetup{table-format=1.2e-1, table-number-alignment=center}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l Sz Sz Sz Sz Sz}
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Branin (2)}
    & \multicolumn{2}{c}{\bfseries Eggholder (2)}
    & \multicolumn{2}{c}{\bfseries GoldsteinPrice (2)}
    & \multicolumn{2}{c}{\bfseries SixHumpCamel (2)}
    & \multicolumn{2}{c}{\bfseries Hartmann3 (3)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 3.51e-02 & \best 3.14e-02 &  \best 8.61e+01 & \best 3.75e+01 &  \statsimilar 4.74e+00 & \statsimilar 6.11e+00 &  \best 2.58e-02 & \best 2.02e-02 &  \best 4.68e-03 & \best 2.85e-03 \\
    MCMC &  8.47e-02 & 9.31e-02 &  \statsimilar 1.02e+02 & \statsimilar 5.17e+01 &  \best 4.07e+00 & \best 5.72e+00 &  4.84e-02 & 4.47e-02 &  9.81e-03 & 2.12e-03 \\
    MFVI &  9.01e-02 & 9.74e-02 &  \statsimilar 9.00e+01 & \statsimilar 4.54e+01 &  \statsimilar 7.22e+00 & \statsimilar 6.37e+00 &  \statsimilar 3.64e-02 & \statsimilar 2.84e-02 &  1.11e-02 & 3.70e-03 \\
    FRVI &  9.60e-02 & 1.08e-01 &  \statsimilar 1.02e+02 & \statsimilar 4.61e+01 &  \statsimilar 4.71e+00 & \statsimilar 4.87e+00 &  \statsimilar 2.84e-02 & \statsimilar 2.37e-02 &  1.04e-02 & 3.00e-03 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Ackley5 (5)}
    & \multicolumn{2}{c}{\bfseries Michalewicz5 (5)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang5 (5)}
    & \multicolumn{2}{c}{\bfseries Hartmann6 (6)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock7 (7)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 4.36e+00 & \best 6.15e-01 &  \best 1.71e+00 & \best 4.53e-01 &  \best 5.25e+01 & \best 1.67e+01 &  \best 3.40e-02 & \best 2.18e-02 &  1.04e+04 & 7.73e+03 \\
    MCMC &  7.05e+00 & 2.02e+00 &  2.25e+00 & 3.26e-01 &  7.73e+01 & 1.36e+01 &  1.97e-01 & 6.65e-02 &  \best 3.46e+03 & \best 3.40e+03 \\
    MFVI &  7.61e+00 & 1.33e+00 &  2.15e+00 & 2.88e-01 &  7.58e+01 & 1.32e+01 &  2.15e-01 & 4.29e-02 &  \statsimilar 4.97e+03 & \statsimilar 5.00e+03 \\
    FRVI &  6.73e+00 & 1.64e+00 &  2.25e+00 & 2.59e-01 &  7.15e+01 & 1.46e+01 &  2.17e-01 & 4.96e-02 &  \statsimilar 4.87e+03 & \statsimilar 5.13e+03 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries StyblinskiTang7 (7)}
    & \multicolumn{2}{c}{\bfseries Ackley10 (10)}
    & \multicolumn{2}{c}{\bfseries Michalewicz10 (10)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock10 (10)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang10 (10)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 7.08e+01 & \best 2.18e+01 &  \best 1.07e+01 & \best 3.55e+00 &  \best 5.14e+00 & \best 5.68e-01 &  \best 2.16e+04 & \best 1.60e+04 &  \best 1.16e+02 & \best 1.60e+01 \\
    MCMC &  1.21e+02 & 1.99e+01 &  1.81e+01 & 2.87e+00 &  5.49e+00 & 4.99e-01 &  5.86e+04 & 2.61e+04 &  1.35e+02 & 3.11e+01 \\
    MFVI &  1.19e+02 & 1.72e+01 &  1.94e+01 & 1.47e+00 &  5.62e+00 & 5.55e-01 &  6.75e+04 & 1.40e+04 &  1.62e+02 & 3.33e+01 \\
    FRVI &  1.21e+02 & 1.96e+01 &  1.82e+01 & 3.25e+00 &  5.61e+00 & 4.02e-01 &  6.75e+04 & 2.00e+04 &  1.43e+02 & 2.09e+01 \\
\bottomrule
\end{tabular}
}%
\caption{Tabulated results for the UCB acquisition function using an ARD kernel on the $\sigma_n = 0.05$ problems. The median log simple regret and the median absolute deviation from the median (MAD) is shown in the left- and right-hand columns respectively. The method with the lowest median performance is shown in dark grey, with those that are statistically equivalent shown in light grey.}
\label{tbl:ucb:noise=0.05:ARD}
\end{table}

==> includes/noise=0.05_isotropic_ei.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{2pt}
\sisetup{table-format=1.2e-1, table-number-alignment=center}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l Sz Sz Sz Sz Sz}
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Branin (2)}
    & \multicolumn{2}{c}{\bfseries Eggholder (2)}
    & \multicolumn{2}{c}{\bfseries GoldsteinPrice (2)}
    & \multicolumn{2}{c}{\bfseries SixHumpCamel (2)}
    & \multicolumn{2}{c}{\bfseries Hartmann3 (3)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \statsimilar 1.13e-01 & \statsimilar 1.23e-01 &  \statsimilar 7.00e+01 & \statsimilar 7.18e+00 &  \statsimilar 6.13e+00 & \statsimilar 6.38e+00 &  \best 2.89e-02 & \best 3.08e-02 &  \statsimilar 4.99e-03 & \statsimilar 3.36e-03 \\
    MCMC &  \statsimilar 1.25e-01 & \statsimilar 8.62e-02 &  \statsimilar 6.91e+01 & \statsimilar 5.47e+00 &  \statsimilar 5.85e+00 & \statsimilar 6.12e+00 &  \statsimilar 2.89e-02 & \statsimilar 2.59e-02 &  \statsimilar 6.23e-03 & \statsimilar 5.33e-03 \\
    MFVI &  \statsimilar 1.60e-01 & \statsimilar 1.18e-01 &  \statsimilar 6.88e+01 & \statsimilar 5.31e+00 &  \best 2.76e+00 & \best 2.68e+00 &  \statsimilar 4.75e-02 & \statsimilar 4.18e-02 &  \best 4.56e-03 & \best 4.72e-03 \\
    FRVI &  \best 8.35e-02 & \best 8.30e-02 &  \best 6.86e+01 & \best 4.62e+00 &  \statsimilar 3.99e+00 & \statsimilar 4.30e+00 &  \statsimilar 3.02e-02 & \statsimilar 2.37e-02 &  \statsimilar 5.28e-03 & \statsimilar 3.99e-03 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Ackley5 (5)}
    & \multicolumn{2}{c}{\bfseries Michalewicz5 (5)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang5 (5)}
    & \multicolumn{2}{c}{\bfseries Hartmann6 (6)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock7 (7)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  5.28e+00 & 2.45e+00 &  1.23e+00 & 7.00e-01 &  \best 3.25e+01 & \best 1.12e+01 &  \statsimilar 7.76e-02 & \statsimilar 7.39e-02 &  2.41e+03 & 1.21e+03 \\
    MCMC &  \statsimilar 4.76e+00 & \statsimilar 1.48e+00 &  \best 1.06e+00 & \best 6.51e-01 &  4.70e+01 & 1.65e+01 &  \statsimilar 9.74e-02 & \statsimilar 1.07e-01 &  \best 6.47e+02 & \best 4.12e+02 \\
    MFVI &  \statsimilar 4.34e+00 & \statsimilar 1.52e+00 &  1.25e+00 & 7.30e-01 &  4.32e+01 & 1.53e+01 &  \statsimilar 8.55e-02 & \statsimilar 7.04e-02 &  \statsimilar 7.13e+02 & \statsimilar 5.01e+02 \\
    FRVI &  \best 3.93e+00 & \best 1.05e+00 &  1.48e+00 & 8.85e-01 &  5.18e+01 & 1.92e+01 &  \best 7.49e-02 & \best 8.28e-02 &  \statsimilar 7.26e+02 & \statsimilar 4.03e+02 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries StyblinskiTang7 (7)}
    & \multicolumn{2}{c}{\bfseries Ackley10 (10)}
    & \multicolumn{2}{c}{\bfseries Michalewicz10 (10)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock10 (10)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang10 (10)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 6.38e+01 & \best 1.89e+01 &  \best 1.46e+01 & \best 2.56e+00 &  \statsimilar 5.32e+00 & \statsimilar 6.37e-01 &  4.70e+03 & 3.20e+03 &  \best 1.25e+02 & \best 1.87e+01 \\
    MCMC &  8.14e+01 & 1.91e+01 &  1.66e+01 & 3.11e+00 &  \statsimilar 5.35e+00 & \statsimilar 6.51e-01 &  \statsimilar 1.70e+03 & \statsimilar 8.40e+02 &  1.35e+02 & 2.58e+01 \\
    MFVI &  8.35e+01 & 2.31e+01 &  1.66e+01 & 3.40e+00 &  \statsimilar 5.39e+00 & \statsimilar 9.63e-01 &  \best 1.36e+03 & \best 7.91e+02 &  1.30e+02 & 2.94e+01 \\
    FRVI &  8.13e+01 & 1.76e+01 &  1.73e+01 & 2.52e+00 &  \best 5.27e+00 & \best 9.27e-01 &  \statsimilar 1.54e+03 & \statsimilar 1.05e+03 &  1.38e+02 & 3.00e+01 \\
\bottomrule
\end{tabular}
}%
\caption{Tabulated results for the EI acquisition function using an isotropic kernel on the $\sigma_n = 0.05$ problems. The median log simple regret and the median absolute deviation from the median (MAD) is shown in the left- and right-hand columns respectively. The method with the lowest median performance is shown in dark grey, with those that are statistically equivalent shown in light grey.}
\label{tbl:ei:noise=0.05:isotropic}
\end{table}

==> includes/noise=0.05_isotropic_ucb.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{2pt}
\sisetup{table-format=1.2e-1, table-number-alignment=center}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l Sz Sz Sz Sz Sz}
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Branin (2)}
    & \multicolumn{2}{c}{\bfseries Eggholder (2)}
    & \multicolumn{2}{c}{\bfseries GoldsteinPrice (2)}
    & \multicolumn{2}{c}{\bfseries SixHumpCamel (2)}
    & \multicolumn{2}{c}{\bfseries Hartmann3 (3)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 8.33e-02 & \best 9.12e-02 &  \statsimilar 8.36e+01 & \statsimilar 3.62e+01 &  \statsimilar 8.09e+00 & \statsimilar 8.18e+00 &  \best 2.95e-02 & \best 2.66e-02 &  \best 5.48e-03 & \best 3.29e-03 \\
    MCMC &  \statsimilar 1.23e-01 & \statsimilar 1.02e-01 &  \best 7.93e+01 & \best 6.09e+01 &  \best 6.20e+00 & \best 7.42e+00 &  4.40e-02 & 3.46e-02 &  1.30e-02 & 8.03e-03 \\
    MFVI &  \statsimilar 1.09e-01 & \statsimilar 8.55e-02 &  \statsimilar 8.45e+01 & \statsimilar 3.46e+01 &  \statsimilar 6.67e+00 & \statsimilar 6.47e+00 &  \statsimilar 4.29e-02 & \statsimilar 5.20e-02 &  1.38e-02 & 1.15e-02 \\
    FRVI &  \statsimilar 1.03e-01 & \statsimilar 1.12e-01 &  \statsimilar 1.01e+02 & \statsimilar 2.94e+01 &  \statsimilar 6.70e+00 & \statsimilar 6.44e+00 &  5.21e-02 & 4.26e-02 &  1.45e-02 & 9.79e-03 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Ackley5 (5)}
    & \multicolumn{2}{c}{\bfseries Michalewicz5 (5)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang5 (5)}
    & \multicolumn{2}{c}{\bfseries Hartmann6 (6)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock7 (7)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 4.23e+00 & \best 8.57e-01 &  \best 1.52e+00 & \best 4.67e-01 &  \best 3.56e+01 & \best 1.28e+01 &  \best 1.03e-01 & \best 1.01e-01 &  \best 2.62e+03 & \best 1.58e+03 \\
    MCMC &  6.64e+00 & 1.52e+00 &  2.35e+00 & 3.48e-01 &  8.14e+01 & 1.46e+01 &  3.51e-01 & 1.55e-01 &  3.97e+03 & 1.10e+03 \\
    MFVI &  6.73e+00 & 1.53e+00 &  2.41e+00 & 3.28e-01 &  8.14e+01 & 1.46e+01 &  3.53e-01 & 2.08e-01 &  3.55e+03 & 1.11e+03 \\
    FRVI &  6.89e+00 & 1.31e+00 &  2.23e+00 & 3.56e-01 &  8.14e+01 & 1.46e+01 &  3.26e-01 & 2.02e-01 &  4.30e+03 & 1.30e+03 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries StyblinskiTang7 (7)}
    & \multicolumn{2}{c}{\bfseries Ackley10 (10)}
    & \multicolumn{2}{c}{\bfseries Michalewicz10 (10)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock10 (10)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang10 (10)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 6.99e+01 & \best 2.02e+01 &  \best 1.26e+01 & \best 5.90e+00 &  \best 5.32e+00 & \best 6.60e-01 &  \statsimilar 1.03e+04 & \statsimilar 7.02e+03 &  \best 1.27e+02 & \best 2.11e+01 \\
    MCMC &  1.22e+02 & 1.92e+01 &  1.93e+01 & 1.68e+00 &  6.26e+00 & 5.45e-01 &  \statsimilar 8.93e+03 & \statsimilar 8.71e+03 &  1.85e+02 & 2.28e+01 \\
    MFVI &  1.21e+02 & 2.00e+01 &  1.86e+01 & 2.71e+00 &  6.09e+00 & 5.46e-01 &  \best 5.13e+03 & \best 3.50e+03 &  1.87e+02 & 2.49e+01 \\
    FRVI &  1.21e+02 & 2.02e+01 &  1.51e+01 & 4.98e+00 &  5.99e+00 & 3.77e-01 &  \statsimilar 8.37e+03 & \statsimilar 7.42e+03 &  1.87e+02 & 2.57e+01 \\
\bottomrule
\end{tabular}
}%
\caption{Tabulated results for the UCB acquisition function using an isotropic kernel on the $\sigma_n = 0.05$ problems. The median log simple regret and the median absolute deviation from the median (MAD) is shown in the left- and right-hand columns respectively. The method with the lowest median performance is shown in dark grey, with those that are statistically equivalent shown in light grey.}
\label{tbl:ucb:noise=0.05:isotropic}
\end{table}

==> includes/noise=0.1_ARD_ei.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{2pt}
\sisetup{table-format=1.2e-1, table-number-alignment=center}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l Sz Sz Sz Sz Sz}
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Branin (2)}
    & \multicolumn{2}{c}{\bfseries Eggholder (2)}
    & \multicolumn{2}{c}{\bfseries GoldsteinPrice (2)}
    & \multicolumn{2}{c}{\bfseries SixHumpCamel (2)}
    & \multicolumn{2}{c}{\bfseries Hartmann3 (3)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 7.02e-02 & \best 7.25e-02 &  \best 5.80e+01 & \best 3.41e+01 &  \statsimilar 7.92e+00 & \statsimilar 7.06e+00 &  \statsimilar 5.01e-02 & \statsimilar 4.60e-02 &  \statsimilar 1.08e-02 & \statsimilar 5.00e-03 \\
    MCMC &  \statsimilar 9.71e-02 & \statsimilar 1.13e-01 &  \statsimilar 6.65e+01 & \statsimilar 1.94e+01 &  \best 6.08e+00 & \best 5.83e+00 &  \best 3.63e-02 & \best 3.66e-02 &  \statsimilar 1.55e-02 & \statsimilar 9.23e-03 \\
    MFVI &  \statsimilar 7.99e-02 & \statsimilar 8.86e-02 &  \statsimilar 6.85e+01 & \statsimilar 5.04e+01 &  \statsimilar 7.19e+00 & \statsimilar 7.36e+00 &  \statsimilar 4.68e-02 & \statsimilar 4.72e-02 &  \best 1.06e-02 & \best 5.45e-03 \\
    FRVI &  \statsimilar 1.11e-01 & \statsimilar 1.12e-01 &  \statsimilar 6.65e+01 & \statsimilar 1.94e+01 &  \statsimilar 7.12e+00 & \statsimilar 8.27e+00 &  \statsimilar 4.57e-02 & \statsimilar 5.04e-02 &  \statsimilar 1.23e-02 & \statsimilar 5.31e-03 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Ackley5 (5)}
    & \multicolumn{2}{c}{\bfseries Michalewicz5 (5)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang5 (5)}
    & \multicolumn{2}{c}{\bfseries Hartmann6 (6)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock7 (7)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \statsimilar 1.07e+01 & \statsimilar 4.29e+00 &  1.95e+00 & 4.00e-01 &  \best 4.07e+01 & \best 9.25e+00 &  \best 1.96e-01 & \best 7.30e-02 &  5.35e+03 & 3.92e+03 \\
    MCMC &  \best 1.00e+01 & \best 3.74e+00 &  \best 1.45e+00 & \best 3.41e-01 &  5.20e+01 & 1.37e+01 &  \statsimilar 1.96e-01 & \statsimilar 6.28e-02 &  \statsimilar 3.06e+03 & \statsimilar 2.22e+03 \\
    MFVI &  \statsimilar 1.13e+01 & \statsimilar 6.27e+00 &  1.75e+00 & 3.71e-01 &  5.50e+01 & 1.16e+01 &  \statsimilar 2.09e-01 & \statsimilar 8.75e-02 &  3.36e+03 & 1.98e+03 \\
    FRVI &  \statsimilar 1.04e+01 & \statsimilar 6.23e+00 &  1.80e+00 & 3.78e-01 &  5.44e+01 & 1.64e+01 &  \statsimilar 2.09e-01 & \statsimilar 4.45e-02 &  \best 2.47e+03 & \best 2.07e+03 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries StyblinskiTang7 (7)}
    & \multicolumn{2}{c}{\bfseries Ackley10 (10)}
    & \multicolumn{2}{c}{\bfseries Michalewicz10 (10)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock10 (10)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang10 (10)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 7.31e+01 & \best 1.09e+01 &  \statsimilar 1.93e+01 & \statsimilar 8.98e-01 &  5.71e+00 & 5.37e-01 &  1.36e+04 & 8.34e+03 &  \best 1.18e+02 & \best 1.83e+01 \\
    MCMC &  8.07e+01 & 2.34e+01 &  \best 1.90e+01 & \best 1.05e+00 &  \best 5.20e+00 & \best 3.79e-01 &  \best 6.53e+03 & \best 3.46e+03 &  1.32e+02 & 2.76e+01 \\
    MFVI &  8.75e+01 & 1.66e+01 &  1.98e+01 & 5.16e-01 &  5.72e+00 & 4.82e-01 &  \statsimilar 7.76e+03 & \statsimilar 3.76e+03 &  \statsimilar 1.25e+02 & \statsimilar 2.27e+01 \\
    FRVI &  8.62e+01 & 1.44e+01 &  \statsimilar 1.95e+01 & \statsimilar 8.24e-01 &  5.68e+00 & 4.39e-01 &  \statsimilar 7.04e+03 & \statsimilar 4.72e+03 &  1.36e+02 & 2.28e+01 \\
\bottomrule
\end{tabular}
}%
\caption{Tabulated results for the EI acquisition function using an ARD kernel on the $\sigma_n = 0.1$ problems. The median log simple regret and the median absolute deviation from the median (MAD) is shown in the left- and right-hand columns respectively. The method with the lowest median performance is shown in dark grey, with those that are statistically equivalent shown in light grey.}
\label{tbl:ei:noise=0.1:ARD}
\end{table}

==> includes/noise=0.1_ARD_ucb.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{2pt}
\sisetup{table-format=1.2e-1, table-number-alignment=center}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l Sz Sz Sz Sz Sz}
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Branin (2)}
    & \multicolumn{2}{c}{\bfseries Eggholder (2)}
    & \multicolumn{2}{c}{\bfseries GoldsteinPrice (2)}
    & \multicolumn{2}{c}{\bfseries SixHumpCamel (2)}
    & \multicolumn{2}{c}{\bfseries Hartmann3 (3)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 3.28e-02 & \best 3.58e-02 &  \best 8.31e+01 & \best 3.21e+01 &  \statsimilar 5.56e+00 & \statsimilar 5.21e+00 &  \best 3.07e-02 & \best 3.72e-02 &  \best 9.47e-03 & \best 3.06e-03 \\
    MCMC &  6.85e-02 & 7.48e-02 &  \statsimilar 8.35e+01 & \statsimilar 4.09e+01 &  \statsimilar 5.60e+00 & \statsimilar 5.91e+00 &  \statsimilar 4.04e-02 & \statsimilar 4.53e-02 &  1.72e-02 & 7.04e-03 \\
    MFVI &  7.32e-02 & 8.50e-02 &  \statsimilar 9.11e+01 & \statsimilar 5.66e+01 &  \statsimilar 5.77e+00 & \statsimilar 4.79e+00 &  \statsimilar 4.08e-02 & \statsimilar 4.86e-02 &  1.45e-02 & 5.84e-03 \\
    FRVI &  7.25e-02 & 7.16e-02 &  \statsimilar 1.01e+02 & \statsimilar 4.46e+01 &  \best 5.22e+00 & \best 6.22e+00 &  \statsimilar 5.07e-02 & \statsimilar 4.34e-02 &  1.44e-02 & 7.01e-03 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Ackley5 (5)}
    & \multicolumn{2}{c}{\bfseries Michalewicz5 (5)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang5 (5)}
    & \multicolumn{2}{c}{\bfseries Hartmann6 (6)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock7 (7)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 7.26e+00 & \best 2.26e+00 &  \best 1.97e+00 & \best 4.00e-01 &  \best 5.44e+01 & \best 1.31e+01 &  \best 2.08e-01 & \best 6.69e-02 &  \statsimilar 7.24e+03 & \statsimilar 5.46e+03 \\
    MCMC &  1.70e+01 & 3.59e+00 &  2.26e+00 & 3.44e-01 &  6.91e+01 & 1.99e+01 &  2.78e-01 & 6.03e-02 &  \statsimilar 9.33e+03 & \statsimilar 7.78e+03 \\
    MFVI &  1.66e+01 & 4.48e+00 &  2.20e+00 & 3.13e-01 &  7.12e+01 & 2.01e+01 &  3.00e-01 & 8.37e-02 &  \best 7.22e+03 & \best 7.60e+03 \\
    FRVI &  1.71e+01 & 3.42e+00 &  2.18e+00 & 3.27e-01 &  7.46e+01 & 1.98e+01 &  2.72e-01 & 3.84e-02 &  \statsimilar 7.33e+03 & \statsimilar 7.13e+03 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries StyblinskiTang7 (7)}
    & \multicolumn{2}{c}{\bfseries Ackley10 (10)}
    & \multicolumn{2}{c}{\bfseries Michalewicz10 (10)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock10 (10)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang10 (10)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 7.14e+01 & \best 1.63e+01 &  \best 1.89e+01 & \best 1.87e+00 &  \best 5.30e+00 & \best 5.98e-01 &  \best 2.86e+04 & \best 2.15e+04 &  \best 1.14e+02 & \best 2.19e+01 \\
    MCMC &  1.11e+02 & 1.30e+01 &  2.01e+01 & 4.59e-01 &  5.66e+00 & 4.59e-01 &  7.07e+04 & 3.47e+04 &  1.23e+02 & 2.68e+01 \\
    MFVI &  1.11e+02 & 2.62e+01 &  2.02e+01 & 3.67e-01 &  6.05e+00 & 5.43e-01 &  6.92e+04 & 3.08e+04 &  1.48e+02 & 2.90e+01 \\
    FRVI &  1.11e+02 & 1.69e+01 &  2.01e+01 & 4.75e-01 &  5.82e+00 & 6.18e-01 &  7.25e+04 & 2.21e+04 &  1.36e+02 & 3.00e+01 \\
\bottomrule
\end{tabular}
}%
\caption{Tabulated results for the UCB acquisition function using an ARD kernel on the $\sigma_n = 0.1$ problems. The median log simple regret and the median absolute deviation from the median (MAD) is shown in the left- and right-hand columns respectively. The method with the lowest median performance is shown in dark grey, with those that are statistically equivalent shown in light grey.}
\label{tbl:ucb:noise=0.1:ARD}
\end{table}

==> includes/noise=0.1_isotropic_ei.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{2pt}
\sisetup{table-format=1.2e-1, table-number-alignment=center}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l Sz Sz Sz Sz Sz}
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Branin (2)}
    & \multicolumn{2}{c}{\bfseries Eggholder (2)}
    & \multicolumn{2}{c}{\bfseries GoldsteinPrice (2)}
    & \multicolumn{2}{c}{\bfseries SixHumpCamel (2)}
    & \multicolumn{2}{c}{\bfseries Hartmann3 (3)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 6.57e-02 & \best 8.76e-02 &  \best 6.84e+01 & \best 2.37e+01 &  \statsimilar 8.07e+00 & \statsimilar 6.88e+00 &  \statsimilar 5.55e-02 & \statsimilar 5.32e-02 &  \statsimilar 1.06e-02 & \statsimilar 8.24e-03 \\
    MCMC &  \statsimilar 1.34e-01 & \statsimilar 9.90e-02 &  \statsimilar 7.11e+01 & \statsimilar 7.75e+00 &  \best 4.64e+00 & \best 5.81e+00 &  \statsimilar 5.66e-02 & \statsimilar 4.23e-02 &  \best 9.60e-03 & \best 7.81e-03 \\
    MFVI &  \statsimilar 9.78e-02 & \statsimilar 9.41e-02 &  \statsimilar 7.13e+01 & \statsimilar 8.22e+00 &  \statsimilar 5.61e+00 & \statsimilar 5.62e+00 &  \best 4.22e-02 & \best 4.07e-02 &  \statsimilar 1.12e-02 & \statsimilar 9.39e-03 \\
    FRVI &  \statsimilar 1.19e-01 & \statsimilar 9.89e-02 &  \statsimilar 6.86e+01 & \statsimilar 1.31e+01 &  \statsimilar 6.46e+00 & \statsimilar 7.15e+00 &  \statsimilar 5.12e-02 & \statsimilar 5.42e-02 &  \statsimilar 1.07e-02 & \statsimilar 6.75e-03 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Ackley5 (5)}
    & \multicolumn{2}{c}{\bfseries Michalewicz5 (5)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang5 (5)}
    & \multicolumn{2}{c}{\bfseries Hartmann6 (6)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock7 (7)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 8.38e+00 & \best 2.74e+00 &  \best 1.32e+00 & \best 6.33e-01 &  \best 4.49e+01 & \best 1.29e+01 &  \statsimilar 2.11e-01 & \statsimilar 1.22e-01 &  3.10e+03 & 2.32e+03 \\
    MCMC &  9.67e+00 & 6.68e+00 &  \statsimilar 1.54e+00 & \statsimilar 6.38e-01 &  5.35e+01 & 1.08e+01 &  \statsimilar 2.20e-01 & \statsimilar 8.51e-02 &  \best 9.78e+02 & \best 9.02e+02 \\
    MFVI &  \statsimilar 9.12e+00 & \statsimilar 3.75e+00 &  1.95e+00 & 7.21e-01 &  5.94e+01 & 1.73e+01 &  \statsimilar 2.13e-01 & \statsimilar 1.22e-01 &  \statsimilar 1.29e+03 & \statsimilar 1.01e+03 \\
    FRVI &  \statsimilar 9.46e+00 & \statsimilar 6.85e+00 &  1.79e+00 & 5.52e-01 &  5.62e+01 & 1.63e+01 &  \best 2.01e-01 & \best 8.47e-02 &  \statsimilar 1.13e+03 & \statsimilar 9.01e+02 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries StyblinskiTang7 (7)}
    & \multicolumn{2}{c}{\bfseries Ackley10 (10)}
    & \multicolumn{2}{c}{\bfseries Michalewicz10 (10)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock10 (10)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang10 (10)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 6.96e+01 & \best 1.89e+01 &  \best 1.69e+01 & \best 1.56e+00 &  \best 5.78e+00 & \best 2.93e-01 &  3.98e+03 & 2.53e+03 &  \best 1.31e+02 & \best 1.89e+01 \\
    MCMC &  9.68e+01 & 2.36e+01 &  1.89e+01 & 1.25e+00 &  \statsimilar 5.78e+00 & \statsimilar 5.25e-01 &  2.47e+03 & 1.57e+03 &  1.50e+02 & 3.83e+01 \\
    MFVI &  9.75e+01 & 2.45e+01 &  1.96e+01 & 7.46e-01 &  \statsimilar 5.96e+00 & \statsimilar 4.30e-01 &  \statsimilar 2.37e+03 & \statsimilar 1.81e+03 &  1.45e+02 & 2.80e+01 \\
    FRVI &  9.52e+01 & 1.95e+01 &  1.94e+01 & 1.04e+00 &  \statsimilar 5.80e+00 & \statsimilar 5.92e-01 &  \best 1.78e+03 & \best 1.39e+03 &  1.46e+02 & 2.82e+01 \\
\bottomrule
\end{tabular}
}%
\caption{Tabulated results for the EI acquisition function using an isotropic kernel on the $\sigma_n = 0.1$ problems. The median log simple regret and the median absolute deviation from the median (MAD) is shown in the left- and right-hand columns respectively. The method with the lowest median performance is shown in dark grey, with those that are statistically equivalent shown in light grey.}
\label{tbl:ei:noise=0.1:isotropic}
\end{table}

==> includes/noise=0.1_isotropic_ucb.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{2pt}
\sisetup{table-format=1.2e-1, table-number-alignment=center}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l Sz Sz Sz Sz Sz}
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Branin (2)}
    & \multicolumn{2}{c}{\bfseries Eggholder (2)}
    & \multicolumn{2}{c}{\bfseries GoldsteinPrice (2)}
    & \multicolumn{2}{c}{\bfseries SixHumpCamel (2)}
    & \multicolumn{2}{c}{\bfseries Hartmann3 (3)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 6.99e-02 & \best 7.82e-02 &  \statsimilar 9.60e+01 & \statsimilar 2.10e+01 &  \statsimilar 6.49e+00 & \statsimilar 7.33e+00 &  \best 3.39e-02 & \best 2.84e-02 &  \best 7.29e-03 & \best 5.50e-03 \\
    MCMC &  \statsimilar 1.03e-01 & \statsimilar 1.01e-01 &  \statsimilar 1.02e+02 & \statsimilar 2.74e+01 &  \statsimilar 8.04e+00 & \statsimilar 8.45e+00 &  \statsimilar 4.27e-02 & \statsimilar 2.60e-02 &  1.93e-02 & 1.50e-02 \\
    MFVI &  \statsimilar 1.24e-01 & \statsimilar 1.30e-01 &  \best 8.84e+01 & \best 3.39e+01 &  \statsimilar 8.84e+00 & \statsimilar 8.22e+00 &  \statsimilar 5.39e-02 & \statsimilar 4.41e-02 &  1.28e-02 & 7.39e-03 \\
    FRVI &  \statsimilar 1.18e-01 & \statsimilar 1.01e-01 &  \statsimilar 1.01e+02 & \statsimilar 3.15e+01 &  \best 4.91e+00 & \best 5.99e+00 &  \statsimilar 3.81e-02 & \statsimilar 4.66e-02 &  1.43e-02 & 7.29e-03 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Ackley5 (5)}
    & \multicolumn{2}{c}{\bfseries Michalewicz5 (5)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang5 (5)}
    & \multicolumn{2}{c}{\bfseries Hartmann6 (6)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock7 (7)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 7.63e+00 & \best 2.57e+00 &  \best 1.61e+00 & \best 5.03e-01 &  \best 4.51e+01 & \best 1.69e+01 &  \best 1.96e-01 & \best 1.31e-01 &  \best 2.34e+03 & \best 2.11e+03 \\
    MCMC &  1.85e+01 & 2.51e+00 &  2.32e+00 & 4.83e-01 &  8.01e+01 & 2.09e+01 &  4.93e-01 & 1.53e-01 &  4.74e+03 & 2.77e+03 \\
    MFVI &  1.93e+01 & 1.51e+00 &  2.27e+00 & 3.39e-01 &  7.80e+01 & 2.25e+01 &  4.35e-01 & 2.06e-01 &  4.60e+03 & 2.30e+03 \\
    FRVI &  1.85e+01 & 2.46e+00 &  2.42e+00 & 4.38e-01 &  8.01e+01 & 2.17e+01 &  3.55e-01 & 1.99e-01 &  4.52e+03 & 1.90e+03 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries StyblinskiTang7 (7)}
    & \multicolumn{2}{c}{\bfseries Ackley10 (10)}
    & \multicolumn{2}{c}{\bfseries Michalewicz10 (10)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock10 (10)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang10 (10)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 7.94e+01 & \best 1.51e+01 &  \best 1.81e+01 & \best 2.33e+00 &  \best 5.39e+00 & \best 4.79e-01 &  \best 1.01e+04 & \best 5.67e+03 &  \best 1.31e+02 & \best 2.64e+01 \\
    MCMC &  1.17e+02 & 1.94e+01 &  2.01e+01 & 4.37e-01 &  6.22e+00 & 4.73e-01 &  6.08e+04 & 1.12e+04 &  1.90e+02 & 3.31e+01 \\
    MFVI &  1.17e+02 & 2.13e+01 &  2.01e+01 & 4.36e-01 &  6.23e+00 & 5.84e-01 &  6.10e+04 & 1.03e+04 &  1.84e+02 & 3.17e+01 \\
    FRVI &  1.17e+02 & 2.12e+01 &  2.02e+01 & 3.75e-01 &  6.18e+00 & 6.00e-01 &  6.19e+04 & 1.39e+04 &  1.90e+02 & 3.87e+01 \\
\bottomrule
\end{tabular}
}%
\caption{Tabulated results for the UCB acquisition function using an isotropic kernel on the $\sigma_n = 0.1$ problems. The median log simple regret and the median absolute deviation from the median (MAD) is shown in the left- and right-hand columns respectively. The method with the lowest median performance is shown in dark grey, with those that are statistically equivalent shown in light grey.}
\label{tbl:ucb:noise=0.1:isotropic}
\end{table}

==> includes/noise=0.2_ARD_ei.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{2pt}
\sisetup{table-format=1.2e-1, table-number-alignment=center}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l Sz Sz Sz Sz Sz}
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Branin (2)}
    & \multicolumn{2}{c}{\bfseries Eggholder (2)}
    & \multicolumn{2}{c}{\bfseries GoldsteinPrice (2)}
    & \multicolumn{2}{c}{\bfseries SixHumpCamel (2)}
    & \multicolumn{2}{c}{\bfseries Hartmann3 (3)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \statsimilar 2.71e-01 & \statsimilar 2.46e-01 &  \statsimilar 8.47e+01 & \statsimilar 2.48e+01 &  \statsimilar 8.11e+00 & \statsimilar 7.32e+00 &  \statsimilar 4.90e-02 & \statsimilar 4.46e-02 &  2.00e-02 & 1.66e-02 \\
    MCMC &  \best 1.46e-01 & \best 1.72e-01 &  \statsimilar 7.44e+01 & \statsimilar 3.92e+01 &  \statsimilar 7.33e+00 & \statsimilar 6.41e+00 &  \statsimilar 7.22e-02 & \statsimilar 5.93e-02 &  \statsimilar 1.82e-02 & \statsimilar 1.36e-02 \\
    MFVI &  \statsimilar 1.50e-01 & \statsimilar 1.60e-01 &  \statsimilar 7.62e+01 & \statsimilar 3.94e+01 &  \statsimilar 9.91e+00 & \statsimilar 1.02e+01 &  \statsimilar 5.26e-02 & \statsimilar 5.71e-02 &  2.14e-02 & 1.59e-02 \\
    FRVI &  \statsimilar 1.65e-01 & \statsimilar 1.56e-01 &  \best 7.15e+01 & \best 4.63e+01 &  \best 6.98e+00 & \best 8.20e+00 &  \best 4.75e-02 & \best 4.08e-02 &  \best 1.48e-02 & \best 6.87e-03 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Ackley5 (5)}
    & \multicolumn{2}{c}{\bfseries Michalewicz5 (5)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang5 (5)}
    & \multicolumn{2}{c}{\bfseries Hartmann6 (6)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock7 (7)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \statsimilar 1.80e+01 & \statsimilar 2.56e+00 &  2.31e+00 & 4.71e-01 &  \best 4.32e+01 & \best 1.81e+01 &  \statsimilar 2.85e-01 & \statsimilar 1.33e-01 &  \statsimilar 1.12e+04 & \statsimilar 7.99e+03 \\
    MCMC &  \best 1.61e+01 & \best 2.91e+00 &  \best 1.93e+00 & \best 4.56e-01 &  \statsimilar 5.57e+01 & \statsimilar 1.15e+01 &  \statsimilar 2.73e-01 & \statsimilar 8.93e-02 &  \best 7.69e+03 & \best 6.05e+03 \\
    MFVI &  \statsimilar 1.71e+01 & \statsimilar 3.26e+00 &  \statsimilar 2.08e+00 & \statsimilar 3.77e-01 &  \statsimilar 5.50e+01 & \statsimilar 1.66e+01 &  \statsimilar 3.07e-01 & \statsimilar 1.08e-01 &  \statsimilar 1.20e+04 & \statsimilar 1.10e+04 \\
    FRVI &  1.81e+01 & 2.06e+00 &  2.11e+00 & 3.18e-01 &  5.55e+01 & 1.58e+01 &  \best 2.62e-01 & \best 9.05e-02 &  \statsimilar 1.19e+04 & \statsimilar 1.14e+04 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries StyblinskiTang7 (7)}
    & \multicolumn{2}{c}{\bfseries Ackley10 (10)}
    & \multicolumn{2}{c}{\bfseries Michalewicz10 (10)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock10 (10)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang10 (10)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 7.40e+01 & \best 1.85e+01 &  \statsimilar 1.95e+01 & \statsimilar 8.59e-01 &  6.11e+00 & 3.79e-01 &  \best 2.59e+04 & \best 1.16e+04 &  \best 1.27e+02 & \best 2.12e+01 \\
    MCMC &  9.05e+01 & 2.22e+01 &  \best 1.92e+01 & \best 6.95e-01 &  \best 5.97e+00 & \best 5.23e-01 &  3.36e+04 & 3.07e+04 &  \statsimilar 1.33e+02 & \statsimilar 3.37e+01 \\
    MFVI &  8.12e+01 & 1.55e+01 &  1.97e+01 & 7.00e-01 &  6.06e+00 & 4.34e-01 &  3.18e+04 & 2.82e+04 &  \statsimilar 1.40e+02 & \statsimilar 2.36e+01 \\
    FRVI &  9.23e+01 & 1.44e+01 &  \statsimilar 1.96e+01 & \statsimilar 8.20e-01 &  \statsimilar 6.04e+00 & \statsimilar 5.06e-01 &  3.22e+04 & 3.38e+04 &  \statsimilar 1.38e+02 & \statsimilar 2.76e+01 \\
\bottomrule
\end{tabular}
}%
\caption{Tabulated results for the EI acquisition function using an ARD kernel on the $\sigma_n = 0.2$ problems. The median log simple regret and the median absolute deviation from the median (MAD) is shown in the left- and right-hand columns respectively. The method with the lowest median performance is shown in dark grey, with those that are statistically equivalent shown in light grey.}
\label{tbl:ei:noise=0.2:ARD}
\end{table}

==> includes/noise=0.2_ARD_ucb.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{2pt}
\sisetup{table-format=1.2e-1, table-number-alignment=center}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l Sz Sz Sz Sz Sz}
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Branin (2)}
    & \multicolumn{2}{c}{\bfseries Eggholder (2)}
    & \multicolumn{2}{c}{\bfseries GoldsteinPrice (2)}
    & \multicolumn{2}{c}{\bfseries SixHumpCamel (2)}
    & \multicolumn{2}{c}{\bfseries Hartmann3 (3)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \statsimilar 2.06e-01 & \statsimilar 2.63e-01 &  \statsimilar 1.01e+02 & \statsimilar 3.75e+01 &  \best 6.62e+00 & \best 7.14e+00 &  \best 1.86e-02 & \best 2.22e-02 &  \best 1.43e-02 & \best 7.74e-03 \\
    MCMC &  \statsimilar 1.96e-01 & \statsimilar 1.88e-01 &  \best 8.62e+01 & \best 4.28e+01 &  \statsimilar 8.83e+00 & \statsimilar 7.79e+00 &  \statsimilar 3.54e-02 & \statsimilar 3.72e-02 &  2.72e-02 & 1.70e-02 \\
    MFVI &  \statsimilar 1.87e-01 & \statsimilar 1.94e-01 &  \statsimilar 1.02e+02 & \statsimilar 1.77e+01 &  \statsimilar 7.54e+00 & \statsimilar 6.96e+00 &  \statsimilar 4.77e-02 & \statsimilar 4.59e-02 &  2.15e-02 & 1.46e-02 \\
    FRVI &  \best 1.39e-01 & \best 1.67e-01 &  \statsimilar 1.01e+02 & \statsimilar 1.91e+01 &  \statsimilar 7.66e+00 & \statsimilar 7.30e+00 &  7.25e-02 & 7.45e-02 &  2.21e-02 & 1.65e-02 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Ackley5 (5)}
    & \multicolumn{2}{c}{\bfseries Michalewicz5 (5)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang5 (5)}
    & \multicolumn{2}{c}{\bfseries Hartmann6 (6)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock7 (7)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 1.78e+01 & \best 2.29e+00 &  \best 2.05e+00 & \best 4.24e-01 &  \best 5.26e+01 & \best 1.54e+01 &  \best 3.34e-01 & \best 1.73e-01 &  \best 1.32e+04 & \best 1.02e+04 \\
    MCMC &  1.88e+01 & 1.70e+00 &  \statsimilar 2.23e+00 & \statsimilar 2.89e-01 &  6.87e+01 & 1.36e+01 &  5.28e-01 & 1.77e-01 &  3.06e+04 & 2.63e+04 \\
    MFVI &  \statsimilar 1.80e+01 & \statsimilar 1.70e+00 &  2.35e+00 & 4.20e-01 &  6.86e+01 & 2.22e+01 &  5.40e-01 & 1.18e-01 &  2.66e+04 & 2.76e+04 \\
    FRVI &  1.86e+01 & 1.77e+00 &  2.38e+00 & 2.72e-01 &  6.88e+01 & 2.25e+01 &  4.52e-01 & 1.72e-01 &  2.71e+04 & 2.27e+04 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries StyblinskiTang7 (7)}
    & \multicolumn{2}{c}{\bfseries Ackley10 (10)}
    & \multicolumn{2}{c}{\bfseries Michalewicz10 (10)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock10 (10)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang10 (10)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 8.12e+01 & \best 1.37e+01 &  \best 1.92e+01 & \best 1.48e+00 &  \best 5.76e+00 & \best 6.10e-01 &  \best 3.99e+04 & \best 3.54e+04 &  \statsimilar 1.30e+02 & \statsimilar 1.98e+01 \\
    MCMC &  1.17e+02 & 2.93e+01 &  2.01e+01 & 5.44e-01 &  \statsimilar 5.94e+00 & \statsimilar 6.28e-01 &  8.18e+04 & 4.87e+04 &  \statsimilar 1.34e+02 & \statsimilar 2.84e+01 \\
    MFVI &  1.17e+02 & 2.67e+01 &  2.02e+01 & 5.70e-01 &  6.32e+00 & 4.60e-01 &  8.53e+04 & 5.07e+04 &  1.56e+02 & 2.55e+01 \\
    FRVI &  1.17e+02 & 2.22e+01 &  2.00e+01 & 6.05e-01 &  6.24e+00 & 5.56e-01 &  9.40e+04 & 5.61e+04 &  \best 1.28e+02 & \best 2.26e+01 \\
\bottomrule
\end{tabular}
}%
\caption{Tabulated results for the UCB acquisition function using an ARD kernel on the $\sigma_n = 0.2$ problems. The median log simple regret and the median absolute deviation from the median (MAD) is shown in the left- and right-hand columns respectively. The method with the lowest median performance is shown in dark grey, with those that are statistically equivalent shown in light grey.}
\label{tbl:ucb:noise=0.2:ARD}
\end{table}

==> includes/noise=0.2_isotropic_ei.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{2pt}
\sisetup{table-format=1.2e-1, table-number-alignment=center}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l Sz Sz Sz Sz Sz}
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Branin (2)}
    & \multicolumn{2}{c}{\bfseries Eggholder (2)}
    & \multicolumn{2}{c}{\bfseries GoldsteinPrice (2)}
    & \multicolumn{2}{c}{\bfseries SixHumpCamel (2)}
    & \multicolumn{2}{c}{\bfseries Hartmann3 (3)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  2.88e-01 & 3.05e-01 &  \statsimilar 7.78e+01 & \statsimilar 3.45e+01 &  \best 3.66e+00 & \best 4.43e+00 &  \statsimilar 6.64e-02 & \statsimilar 5.79e-02 &  \statsimilar 1.87e-02 & \statsimilar 1.34e-02 \\
    MCMC &  \statsimilar 1.72e-01 & \statsimilar 1.56e-01 &  \best 7.32e+01 & \best 3.85e+01 &  8.02e+00 & 7.53e+00 &  \best 3.36e-02 & \best 3.62e-02 &  \best 1.36e-02 & \best 1.31e-02 \\
    MFVI &  \statsimilar 2.05e-01 & \statsimilar 1.78e-01 &  \statsimilar 8.05e+01 & \statsimilar 3.18e+01 &  9.94e+00 & 8.95e+00 &  \statsimilar 6.17e-02 & \statsimilar 5.99e-02 &  \statsimilar 1.95e-02 & \statsimilar 1.59e-02 \\
    FRVI &  \best 1.62e-01 & \best 1.76e-01 &  \statsimilar 7.32e+01 & \statsimilar 4.33e+01 &  \statsimilar 5.94e+00 & \statsimilar 5.95e+00 &  \statsimilar 5.47e-02 & \statsimilar 5.31e-02 &  \statsimilar 2.28e-02 & \statsimilar 1.88e-02 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Ackley5 (5)}
    & \multicolumn{2}{c}{\bfseries Michalewicz5 (5)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang5 (5)}
    & \multicolumn{2}{c}{\bfseries Hartmann6 (6)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock7 (7)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 1.31e+01 & \best 5.57e+00 &  \best 1.88e+00 & \best 5.17e-01 &  \best 4.27e+01 & \best 1.62e+01 &  \statsimilar 3.43e-01 & \statsimilar 1.74e-01 &  7.68e+03 & 5.75e+03 \\
    MCMC &  1.86e+01 & 2.03e+00 &  \statsimilar 1.90e+00 & \statsimilar 5.53e-01 &  6.88e+01 & 1.75e+01 &  \statsimilar 2.84e-01 & \statsimilar 1.38e-01 &  \statsimilar 5.85e+03 & \statsimilar 4.67e+03 \\
    MFVI &  1.89e+01 & 1.55e+00 &  2.20e+00 & 4.81e-01 &  6.62e+01 & 1.28e+01 &  \best 2.70e-01 & \best 1.45e-01 &  \statsimilar 5.60e+03 & \statsimilar 4.73e+03 \\
    FRVI &  1.87e+01 & 1.89e+00 &  2.12e+00 & 5.03e-01 &  6.62e+01 & 1.35e+01 &  \statsimilar 3.14e-01 & \statsimilar 1.51e-01 &  \best 4.98e+03 & \best 4.24e+03 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries StyblinskiTang7 (7)}
    & \multicolumn{2}{c}{\bfseries Ackley10 (10)}
    & \multicolumn{2}{c}{\bfseries Michalewicz10 (10)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock10 (10)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang10 (10)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 7.42e+01 & \best 2.07e+01 &  \best 1.80e+01 & \best 1.52e+00 &  \statsimilar 6.01e+00 & \statsimilar 4.62e-01 &  2.09e+04 & 1.27e+04 &  \best 1.33e+02 & \best 1.82e+01 \\
    MCMC &  1.00e+02 & 2.39e+01 &  1.91e+01 & 8.98e-01 &  6.15e+00 & 3.95e-01 &  \statsimilar 9.54e+03 & \statsimilar 7.34e+03 &  1.67e+02 & 2.16e+01 \\
    MFVI &  1.01e+02 & 2.11e+01 &  1.95e+01 & 9.06e-01 &  6.10e+00 & 4.92e-01 &  \best 6.07e+03 & \best 5.52e+03 &  1.65e+02 & 1.86e+01 \\
    FRVI &  9.24e+01 & 2.42e+01 &  1.94e+01 & 9.59e-01 &  \best 5.86e+00 & \best 4.64e-01 &  \statsimilar 8.90e+03 & \statsimilar 8.74e+03 &  1.60e+02 & 3.02e+01 \\
\bottomrule
\end{tabular}
}%
\caption{Tabulated results for the EI acquisition function using an isotropic kernel on the $\sigma_n = 0.2$ problems. The median log simple regret and the median absolute deviation from the median (MAD) is shown in the left- and right-hand columns respectively. The method with the lowest median performance is shown in dark grey, with those that are statistically equivalent shown in light grey.}
\label{tbl:ei:noise=0.2:isotropic}
\end{table}

==> includes/noise=0.2_isotropic_ucb.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{2pt}
\sisetup{table-format=1.2e-1, table-number-alignment=center}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l Sz Sz Sz Sz Sz}
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Branin (2)}
    & \multicolumn{2}{c}{\bfseries Eggholder (2)}
    & \multicolumn{2}{c}{\bfseries GoldsteinPrice (2)}
    & \multicolumn{2}{c}{\bfseries SixHumpCamel (2)}
    & \multicolumn{2}{c}{\bfseries Hartmann3 (3)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 2.48e-01 & \best 3.04e-01 &  \statsimilar 9.33e+01 & \statsimilar 3.61e+01 &  \statsimilar 5.75e+00 & \statsimilar 7.43e+00 &  \best 3.75e-02 & \best 3.72e-02 &  \best 1.41e-02 & \best 1.17e-02 \\
    MCMC &  \statsimilar 3.07e-01 & \statsimilar 2.65e-01 &  \statsimilar 7.92e+01 & \statsimilar 5.58e+01 &  \statsimilar 3.84e+00 & \statsimilar 4.42e+00 &  \statsimilar 6.21e-02 & \statsimilar 5.73e-02 &  3.16e-02 & 2.02e-02 \\
    MFVI &  \statsimilar 3.77e-01 & \statsimilar 3.43e-01 &  \best 7.28e+01 & \best 5.10e+01 &  \statsimilar 5.73e+00 & \statsimilar 5.09e+00 &  \statsimilar 4.21e-02 & \statsimilar 4.39e-02 &  2.19e-02 & 1.80e-02 \\
    FRVI &  \statsimilar 4.42e-01 & \statsimilar 4.44e-01 &  \statsimilar 8.51e+01 & \statsimilar 4.13e+01 &  \best 2.75e+00 & \best 2.98e+00 &  7.65e-02 & 7.36e-02 &  2.25e-02 & 1.74e-02 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries Ackley5 (5)}
    & \multicolumn{2}{c}{\bfseries Michalewicz5 (5)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang5 (5)}
    & \multicolumn{2}{c}{\bfseries Hartmann6 (6)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock7 (7)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 1.08e+01 & \best 6.89e+00 &  \best 1.89e+00 & \best 4.77e-01 &  \best 4.54e+01 & \best 1.55e+01 &  \best 4.04e-01 & \best 1.67e-01 &  \best 6.51e+03 & \best 6.57e+03 \\
    MCMC &  1.93e+01 & 1.02e+00 &  2.60e+00 & 4.37e-01 &  8.71e+01 & 1.96e+01 &  5.76e-01 & 2.64e-01 &  2.66e+04 & 3.09e+04 \\
    MFVI &  1.93e+01 & 1.22e+00 &  2.65e+00 & 2.64e-01 &  8.67e+01 & 1.99e+01 &  \statsimilar 5.30e-01 & \statsimilar 1.67e-01 &  1.49e+04 & 1.62e+04 \\
    FRVI &  1.93e+01 & 1.15e+00 &  2.74e+00 & 3.22e-01 &  8.67e+01 & 1.99e+01 &  \statsimilar 5.22e-01 & \statsimilar 1.43e-01 &  3.00e+04 & 3.37e+04 \\
\bottomrule
\toprule
    \bfseries Method
    & \multicolumn{2}{c}{\bfseries StyblinskiTang7 (7)}
    & \multicolumn{2}{c}{\bfseries Ackley10 (10)}
    & \multicolumn{2}{c}{\bfseries Michalewicz10 (10)}
    & \multicolumn{2}{c}{\bfseries Rosenbrock10 (10)}
    & \multicolumn{2}{c}{\bfseries StyblinskiTang10 (10)} \\
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD}
    & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{MAD} \\ \midrule
    MAP &  \best 7.41e+01 & \best 2.02e+01 &  \best 1.90e+01 & \best 1.15e+00 &  \best 5.62e+00 & \best 3.93e-01 &  \best 4.68e+04 & \best 3.88e+04 &  \best 1.25e+02 & \best 3.15e+01 \\
    MCMC &  1.28e+02 & 2.19e+01 &  2.01e+01 & 5.79e-01 &  6.30e+00 & 5.92e-01 &  8.89e+04 & 5.54e+04 &  1.80e+02 & 2.87e+01 \\
    MFVI &  1.26e+02 & 1.99e+01 &  2.01e+01 & 5.77e-01 &  6.39e+00 & 5.01e-01 &  9.25e+04 & 3.86e+04 &  1.79e+02 & 2.77e+01 \\
    FRVI &  1.26e+02 & 2.08e+01 &  1.99e+01 & 6.47e-01 &  6.33e+00 & 6.01e-01 &  9.25e+04 & 3.73e+04 &  1.81e+02 & 2.29e+01 \\
\bottomrule
\end{tabular}
}%
\caption{Tabulated results for the UCB acquisition function using an isotropic kernel on the $\sigma_n = 0.2$ problems. The median log simple regret and the median absolute deviation from the median (MAD) is shown in the left- and right-hand columns respectively. The method with the lowest median performance is shown in dark grey, with those that are statistically equivalent shown in light grey.}
\label{tbl:ucb:noise=0.2:isotropic}
\end{table}
